Learning to Detect Every Thing in an Open World

Many open-world applications require the detection of novel objects, yet state-of-the-art object detection and instance segmentation networks do not excel at this task. The key issue lies in their assumption that regions without any annotations should be suppressed as negatives, which teaches the model to treat the unannotated objects as background. To address this issue, we propose a simple yet surprisingly powerful data augmentation and training scheme we call Learning to Detect Every Thing (LDET). To avoid suppressing hidden objects, background objects that are visible but unlabeled, we paste annotated objects on a background image sampled from a small region of the original image. Since training solely on such synthetically-augmented images suffers from domain shift, we decouple the training into two parts: 1) training the region classification and regression head on augmented images, and 2)~training the mask heads on original images. In this way, a model does not learn to classify hidden objects as background while generalizing well to real images. LDET leads to significant improvements on many datasets in the open-world instance segmentation task, outperforming baselines on cross-category generalization on COCO, as well as cross-dataset evaluation on UVO and Cityscapes.

==> figures/detected_results_uvo.tex <==
\begin{figure*}[t]
    \centering
    
    \includegraphics[width=\linewidth]{images/detected_results_uvo.pdf}
    \vspace{-2mm}
    \caption{\small{\textbf{Visualization of results for UVO dataset. Top: Mask RCNN. Bottom: \ours.}}}
    \label{fig:examples_result_uvo}
\end{figure*}

==> figures/overfit.tex <==
\begin{figure}[t]
    \centering
    \vspace{-5mm}
    \includegraphics[width=0.7\linewidth]{images/overfitting.png}
    \vspace{-4mm}
    \caption{\small{\textbf{Baseline MaskRCNN suffers from overfitting to annotated instances.} It thus decreases the performance to detect novel objects as training proceeds. In contrast, our approach basically gains performance with training iterations.}}
    \label{fig:overfit}
\end{figure}

==> tables/agnostic.tex <==
\begin{table}[t]
\centering
\vspace{-4mm}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Box}& \multicolumn{2}{c}{Mask}\\
& { \small{AR10}} &  \small{AR100}  &  \small{AR10}  &  \small{AR100} \\
\hline 
Geodesic~\cite{krahenbuhl2014geodesic} &4.0 & 18.0 & 2.3. & 12.3 \\ 
Rigor~\cite{humayun2014rigor} & - & 13.3 & - &9.4 \\ 
SelectiveSearch~\cite{uijlings2013selective} & 5.2 & 16.3&2.5&9.5\\ 
MCG~\cite{arbelaez2014multiscale} & 10.1 & 24.6&7.7&18.6\\ 
DeepMask~\cite{pinheiro2015learning} & 15.2 & 30.6 & 12.3&23.3\\
\ours & \\
%\\\textbf{30.3}&\textbf{46.0} & \textbf{27.9}&\textbf{40.8}\\ % \textbf{7.6} &  \textbf{10.3} & \textbf{17.0} &   \\
\bottomrule

\end{tabular}}
\caption{\small{\textbf{Comparison to unsupervised methods and DeepMask tested on COCO.} Results of baselines are reported in DeepMask~\cite{pinheiro2015learning}. Note that DeepMask uses VGG~\cite{simonyan2014very} as backbone. \ours and DeepMask are trained on VOC-COCO. }}
\label{tab:unsupervised}
\vspace{-5mm}
\end{table}


==> tables/backbones.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[t]
\centering
\vspace{-3mm}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|c|rr|rr}
\toprule
\multirow{2}{*}{Method}&\multirow{2}{*}{\small{Backbone}} & \multicolumn{2}{c|}{Box}& \multicolumn{2}{c}{Mask}\\
&& {\small{AP}} &    \small{AR100}  &  {\small{AP}} &  \small{AR100}\\
\hline 
MRCNN &Res50&24.8&47.7&19.1&38.1 \\ 
MRCNN & Res101&\textcolor{blue}{\small{(+1.0)}} 25.8&\textcolor{blue}{\small{(-0.1)}} 47.6&\textcolor{blue}{\small{(+1.2)}} 20.3&\textcolor{blue}{\small{(+0.6)}} 38.7\\\hline

\ours&Res50& 26.1&53.1&21.2&43.0\\
\ours & Res101&\textcolor{blue}{\small{(+1.7)}} 27.8&\textcolor{blue}{\small{(+0.1)}} 53.2&\textcolor{blue}{\small{(+1.9)}} 23.1&
\textcolor{blue}{\small{(+1.1)}} 44.1 \\


\bottomrule


\end{tabular}}
\caption{\small{\textbf{ResNet50 vs ResNet101.} ResNet101 tends to perform better than ResNet50, which is more evident in \ours than in Mask RCNN (MRCNN).}}
\label{tab:backbone}\vspace{-4mm}
\end{table}


==> tables/classagnostic.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[t]
\centering
\vspace{-1mm}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|c|ccc|ccc}
\toprule
\multirow{2}{*}{Method}&\multirow{2}{*}{\small{Agnostic}} & \multicolumn{3}{c|}{Box}& \multicolumn{3}{c}{Mask}\\
&& {\small{AP}} & \small{AR10}   & \small{AR100}  &  {\small{AP}} & \small{AR10}  & \small{AR100}\\
\hline 
Plain &&8.7&16.0&20.9&7.0&13.7&	17.7\\
Plain &\checkmark&\textbf{9.0}&\textbf{18.7}&\textbf{21.6}&\textbf{7.3}&\textbf{13.9}&\textbf{18.1}\\\hline 
\ours&& \textbf{10.2}&21.5&34.9&9.0&19.7&31.0\\
\ours &\checkmark&\textbf{10.2}&\textbf{21.8}&\textbf{35.6}&\textbf{9.2}&\textbf{20.2}&\textbf{32.0}\\
\bottomrule
\end{tabular}}

\caption{\small{\textbf{Ablation study for class agnostic training.} Class agnostic training slightly improves performance in both \ours and the plain Mask RCNN.}}
\label{tab:class_agnostic}
\end{table}

==> tables/coco_to_uvo.tex <==
%%%%%%%%%%%%%%% Train on 
\begin{table}[t]
\small

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{crrrr}
\toprule
Method & {\small{AP$_{\text{box}}$}} & \small{AR$_{\text{box}}$}  & {\small{AP$_{\text{mask}}$}} & \small{AR$_{\text{mask}}$}   \\
\hline 
Mask RCNN&24.2&48.5&18.7&38.6\\
Mask RCNN+ & 20.9 & 48.6&15.2&39.0\\
Ours & \textcolor{blue}{(+0.7)}  24.9 &  \textcolor{blue}{(+5.1)} 53.6 &   \textcolor{blue}{(+1.5)} 20.2& \textcolor{blue}{(+4.8)} 43.4\\
\bottomrule

\end{tabular}
\vspace{-2mm}

\caption{\small{\textbf{Results of {COCO} $\rightarrow$ {UVO} generalization.}}}
\label{tab:coco2uvo}
\end{table}


==> tables/coco_to_uvo_detail.tex <==

%%%%%%%%%%%%%%% Train on COCO, test on UVO
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|rrrrr|rrrrr}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{Box}& \multicolumn{5}{c}{Mask}\\
& {\small{AP}} & \small{AR}  & \small{AR$_{\text{small}}$}  & \small{AR$_{\text{medium}}$}  &  \small{AR$_{\text{large}}$}& {\small{AP}} & \small{AR}  & \small{AR$_{\text{small}}$}  & \small{AR$_{\text{medium}}$}  &  \small{AR$_{\text{large}}$} \\
\hline 

Mask RCNN&24.8&47.7&21.9&41.7&60.6&19.1&38.1&19.1&35.0&46.5\\
Mask RCNN+ & 21.3&47.9&21.1&40.8&62.0&15.6&38.6&19.3&34.9&47.6\\
Ours & \textcolor{blue}{\small{(+1.3)}} \textbf{26.1} &   \textcolor{blue}{\small{(+5.9)}} \textbf{53.1} &  \textcolor{blue}{\small{(+6.5)}} \textbf{28.4} &  

\textcolor{blue}{\small{(+6.1)}} \textbf{47.8} & 
\textcolor{blue}{\small{(+4.4)}} \textbf{65.0} &  

\textcolor{blue}{\small{(+2.1)}} \textbf{21.2}& \textcolor{blue}{\small{(+4.9)}} \textbf{43.0}&  \textcolor{blue}{\small{(+6.6)}} \textbf{25.7}& 
\textcolor{blue}{\small{(+6.1)}} \textbf{41.1}&  \textcolor{blue}{\small{(+3.4)} }\textbf{49.9}\\
\bottomrule

\end{tabular}}
\vspace{-2mm}

\caption{\small{\textbf{Results of {COCO} $\rightarrow$ {UVO} generalization.}}}
\label{tab:coco2uvo}
\end{table*}


==> tables/different_arch.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[t]
\centering
%\vspace{-4mm}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c|c|ccccc}
\toprule
\multirow{1}{*}{\small{Detector}}&\multirow{1}{*}{\small{Method}} &AR$_{10}$&AR$_{30}$&AR$_{50}$&AR$_{100}$ \\
\hline  
\multirow{2}{*}{\small{RetinaNet}}&Plain&9.9&14.1&15.7&17.8\\
&\ours&15.3&23.1&26.7&31.0\\\hline
\multirow{2}{*}{\small{TensorMask}}&Plain&10.6&15.7&17.6&19.7\\
&\ours&16.3&23.5&26.8&31.1\\

\bottomrule


\end{tabular}}
\caption{\small{\textbf{.}}}
\label{tab:different_arch} 
\end{table}


==> tables/one_stage.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|rrrrr}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{Box}\\
& {\small{AP}} & \small{AR10}  & \small{AR30}  &  \small{AR50}  &\small{AR100}  \\
\hline %\hline
RetinaNet~\cite{lin2017focal}&\textbf{9.0} & 16.5&21.0&22.9&25.0\\
\ours & 6.8 & \textbf{18.9} & \textbf{26.1} & \textbf{29.2} & \textbf{32.9}\\
\bottomrule

\end{tabular}}
\vspace{-2mm}

\caption{\small{\textbf{Results of {VOC} $\rightarrow$ {Non-VOC} generalization in COCO using RetinaNet as a detector.}}}
\label{tab:one_stage}
\end{table}


==> tables/rpn_roihead.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[t]
\centering
%\vspace{-4mm}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|c|ccccc}
\toprule
\multirow{1}{*}{Method}&\multirow{1}{*}{\small{Detector}} &AR$_{10}$&AR$_{30}$&AR$_{50}$&AR$_{100}$ \\
\hline  

Plain &RPN&11.0&16.3&	19.4&22.9\\
Plain &ROI&8.8&10.4&10.8&10.9\\\hline
\ours&RPN&15.4&\textbf{30.8}&	26.4&30.8\\
\ours &ROI&\textbf{18.2}&\textbf{30.8}&\textbf{28.0}&\textbf{30.8}\\%\textcolor{blue}{\small{(+3.7)}} 10.2&\textcolor{blue}{\small{(+3.3)}} 21.5&\textcolor{blue}{\small{(+2.0)}} 34.8\\

\bottomrule


\end{tabular}}
\caption{\small{\textbf{Comparison between region proposal network and region of interest head. AP and AR of bounding boxes.}}}
\label{tab:rpn_roihead} 
\end{table}


==> tables/swav_compare.tex <==
\begin{table*}[!ht]
\centering
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|rr|rr|rr|rr}
\toprule

\multirow{3}{*}{Method}&\multirow{3}{*}{\small{\makecell{Pre-training  \\ Data}}}& \multirow{3}{*}{\small{\makecell{Pre-training  \\ Method}}}& \multicolumn{4}{c|}{VOC-to-COCO}& \multicolumn{4}{c}{VOC-to-UVO}\\\cline{4-11}
&&&\multicolumn{2}{c|}{Box}& \multicolumn{2}{c|}{Mask}&\multicolumn{2}{c|}{Box}& \multicolumn{2}{c}{Mask}\\
&&& \small{AP} &    \small{AR}  &  \small{AP} &  \small{AR}& \small{AP} &    \small{AR}  &  \small{AP} &  \small{AR}\\
\hline 
MRCNN &None&None&6.1&24.9&4.6&21.5&16.6&\textbf{37.8}&11.3&\textbf{27.7}\\
MRCNN & ImageNet1K& SWAV~\cite{caron2020unsupervised}&7.1&\textbf{25.3}&5.5&\textbf{22.1}&15.8&37.1&10.8&26.5\\
MRCNN &ImageNet1K&Supervised&\textbf{8.9}&20.9&\textbf{7.2}&17.7&\textbf{19.6}&34.8&\textbf{14.6}&25.8\\ 
MRCNN& ImageNet21K& MIIL~\cite{ridnik2021imagenet}&8.8&20.9&7.0&17.9&19.3&35.0&14.4&25.9\\\hline
LDET&None&None&5.7&29.5&4.2&25.2&15.8&42.7&9.9&30.1\\
LDET & ImageNet1K& SWAV~\cite{caron2020unsupervised}&5.5&29.9&4.7&27.1&13.9&41.2&10.6&30.8\\
LDET &ImageNet1K&Supervised & \textbf{10.2}& 34.8&\textbf{9.0}&31.0&\textbf{22.8}&\textbf{48.9}&\textbf{17.9}&\textbf{38.0}\\
LDET & ImageNet21K& MIIL~\cite{ridnik2021imagenet}&9.7&\textbf{35.3}&8.6&\textbf{31.9}&21.3&48.1&17.1&37.6\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\small{\textbf{Comparison of pre-training methods.} Replacing supervised pre-trained model with SWAV (unsupervised) pre-training degrades AP in both training methods. SWAV performs better on AR of Mask RCNN.}}
\label{tab:model_compare}
\end{table*}


==> tables/test_time_parameters.tex <==
%%%%%%%%%%%%%%% Train on VOC, test on Non-VOC
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|cc}
\toprule
\multirow{2}{*}{\small{NMS Threshold}}&\multirow{2}{*}{\small{Num of Boxes}} & \multicolumn{2}{c|}{Box}& \multicolumn{2}{c}{Mask}\\
&   & {\small{AP}}   & \small{AR}  &  {\small{AP}} & \small{AR}\\
\hline 
0.5 & 1000 & 10.5 & 33.3 & 9.3 & 30.3\\
0.7 & 1000 & 10.3 & 34.9 &9.1 & 31.0 \\
0.5 & 2000 & 10.5 & 33.6 & 9.3 & 30.7\\
0.7 & 2000 & 10.2 & 34.8 & 9.0 & 31.0\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\small{\textbf{Study on the threshold for no-maximum suppression and the number of boxes kept after region proposal network.} The last row is the setting used in the main paper.}}
\label{tab:test_hp}\vspace{-3mm}
\end{table}



